Mr. Right: Multimodal Retrieval on Representation of ImaGe witH Text

Multimodal learning is a recent challenge that extends unimodal learning by generalizing its domain to diverse modalities, such as texts, images, or speech. This extension requires models to process and relate information from multiple modalities. In Information Retrieval, traditional retrieval tasks focus on the similarity between unimodal documents and queries, while image-text retrieval hypothesizes that most texts contain the scene context from images. This separation has ignored that real-world queries may involve text content, image captions, or both. To address this, we introduce Multimodal Retrieval on Representation of ImaGe witH Text (Mr. Right), a novel and comprehensive dataset for multimodal retrieval. We utilize the Wikipedia dataset with rich text-image examples and generate three types of text-based queries with different modality information: text-related, image-related, and mixed. To validate the effectiveness of our dataset, we provide a multimodal training paradigm and evaluate previous text retrieval and image retrieval frameworks. The results show that proposed multimodal retrieval can improve retrieval performance, but creating a well-unified document representation with texts and images is still a challenge. We hope Mr. Right allows us to broaden current retrieval systems better and contributes to accelerating the advancement of multimodal learning in the Information Retrieval.

==> Image/fig-spectrum.tex <==
\begin{figure*}[b]
    \centering
    \includegraphics[width=\textwidth]{Image/spectrum.pdf}
    \caption{Distribution of MRR@10 across all testing samples based on our model (METER) results. }
    \label{fig:spectrum}
\end{figure*}


==> Table/Table-ablation-objetives.tex <==
\begin{table*}[t]
\centering
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{cr|rrr|rrr|rrr}

\toprule
& \multirow{2}{*}{Method} & \multicolumn{3}{c|}{text-related query} & \multicolumn{3}{c|}{image-related query} & 
\multicolumn{3}{c}{mixed query} \\
& &  R@1 & R@5 & R@10 &  R@1 & R@5 & R@10 &  R@1 & R@5 & R@10 \\
\midrule

% & BM25 + ALBEF (FT) & 54.5 & 71.4 & 76.8 & 61.9 & 4.6 & 10.5 & 13.9 & 7.1 & 55.9 & 72.8 & 77.4 & 63.2 \\
\multirow{4}{*}{MR} & DQC+DQM+CP &  31.6 & 60.1 & 72.3  &  1.3 & 4.3 & 7.6  &  35.0 & 65.2 & 76.1 \\
& DQC+CP &  17.3 & 45.6 & 59.6 &  0.2 & 1.4 & 2.6  &  24.6 & 55.5 & 68.8 \\
& DQC+DQM & \textbf{32.3} & \textbf{61.1} & \textbf{72.4}  &  \textbf{2.1} & \textbf{6.2} & \textbf{10.8} &  \textbf{38.0} & \textbf{67.2} & \textbf{78.2}\\

\bottomrule

\end{tabular}}
\caption{Retrieval performance across three benchmark tasks with different types of queries. We compare MRR and recall among baselines and our proposed models on TR, IR and MR. ZS is zero-shot, and FT is fine-tuned.}
\label{tab:ablation_obj}
\vspace{-10pt}
\end{center}
\end{table*}

==> Table/Table-related-dataset_temp.tex <==
\begin{table}[t]
\centering
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lll|r|rr|rrr@{}}

\toprule
                    &                          &                 & \multicolumn{1}{c|}{\textbf{Train}}   & \multicolumn{2}{c|}{\textbf{Dev}} & \multicolumn{3}{c}{\textbf{Test}}                         \\
\textbf{Dataset}    & \textbf{Task}            & \textbf{Source} & \multicolumn{1}{c|}{\textbf{\#Pairs}} & \textbf{\#Pairs}    & \textbf{\#Query}    & \textbf{\#Pairs} & \textbf{\#Query} & \textbf{\#Document} \\ \toprule
MS MARCO (Nguyen et al., NIPS 2016)            & Text Retrieval           & Misc.           & 532,761          & ---                 & ---        & ---     & 6,980            & 8,841,823           \\
TREC-NEWS (Soboroff et al., TREC 2018)          & Text Retrieval           & News            & ---              & ---                 & ---        & ---     & 57               & 594,977             \\
HOTPOTQA (Yang et al., EMNLP 2018) & Question Answering & Wikipedia & 170,000          & ---                 & 5,447        & ---     & 7,405           & 5,233,329  \\
NQ (Kwiatkowski et al., TACL 2019) & Question Answering & Wikipedia & 132,803 & --- & --- & --- & 3,452 &  2,681,468 \\
FEVER (Thorne et al., NAACL 2018) & Fact Checking & Wikipedia & 140,085 & --- & 6,666 & --- & 6,666 &  5,416,568 \\
\midrule
SOP (Song et al., CVPR 2016) & Image-to-Image Retrieval & Products & 59,551 & --- & --- &  --- & 11,316 & 60,502 \\
CUB-200-2011 (Wah et al., 2010) & Image-to-Image Retrieval & Birds &  5,864 & --- & --- & --- & 100 & 5,924 \\
$R$Oxford (Radenović et al., CVPR 2018)            & Image-to-Image Retrieval & Landmark          & ---              & ---                 & ---        & ---     & 70               & 4,993                \\
Ukbench (Wang et al., ICCV 2011)          & Image-to-Image Retrieval & Misc.           & ---              & ---                 & ---        & ---   & 2,550              & 10,200                 \\ \midrule
MS COCO (Lin et al., ECCV 2014)        & Image-Text Retrieval     & Misc.           & 118,000          & 5,000               & ---        & 5,000   & ---              & ---                 \\
Conceptual Captions (Sharma et al., ACL 2018) & Image-Text Retrieval     & Misc.           & $\sim$3,300,000  & 2,800               & ---        & 2,300   & ---              & ---                 \\
Flickr30K (Plummer et al., ICCV 2015)           & Image-Text Retrieval     & Flickr          & 30,000           & 1,000                & ---        & 1,000    & ---              & ---                 \\ 
\midrule
Mr. Right (ours)    & Mutlimodal Retrieval     & Wikipedia       & 351,979 / 1,000          & ---                 & ---      & ---     & 2,047            & 806,357 \\
\bottomrule
\end{tabular}}
\vspace{5pt}
\caption{Statistics of datasets in retrieval tasks. Text-to-text retrieval datasets and image-to-image retrieval datasets contain large documents with fewer queries. Image-text retrieval datasets include pairs of data. Mr. Right is the first multimodal retrieval dataset that involves around 35k auto-generated training pairs, 1k human-annotated pairs for fine-tuning, and 2k annotated pairs for testing.}
\label{tab:dataset}
\vspace{-10pt}
\end{center}
\end{table}


